ReToken: Improving Long-Context VLMs with Visual Retrieval Token

Long visual contexts challenge vision-language models: performance degrades as the number of distractors grows, and processing all tokens at once can exceed GPU memory limits. We present RETOKEN, a single learnable embedding that extracts retrieval signals from the VLM's internal representations to select query-relevant visual tokens from the pre-filled KV cache. This enables retrieval within the answering VLM, without a separate retriever or re-encoding. Despite being trained on only a small image-QA dataset, RETOKEN generalizes across image and video benchmarks. On Visual Haystacks, it improves Qwen3VL-8B by 13.4 points and InternVL3.5 by 12.4 points (>20% relative). On LVBench, it transfers zero-shot to long video and improves Qwen3VL-8B by 8.0 points. Thanks to its lightweight design, both training and long-video inference fit on a single H100. Code is available at: https://github.com/avaxiao/ReToken

==> tab/multi_layer.tex <==
\begin{table}[H]
\caption{\textbf{Single-pass inference with multi-layer supervision performs worse than two-pass inference with single-layer supervision.} Qwen3VL-8B.}
\label{tab:multi_layer}
\setlength\tabcolsep{7pt}
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{@{}lcccccccc@{}}
\toprule
Method  & $C=1$ & $C=2$ & $C=3$ & $C=5$ & $C=10$ & $C=20$ & $C=50$ & $C=100$   \\

\midrule

ReKV~\cite{di2025streaming} & 87.8 & 73.0 & 65.5 & 59.5 & 53.8 & 52.2 & 51.2 & 49.9 \\

% \midrule
% \noalign{\vskip 3pt}\cdashline{1-9}\noalign{\vskip 3pt}
% \multicolumn{9}{@{}l}{\textbf{\textcolor{gray}{\texttt{ReToken}}}} \\

% \rowcolor{SeaGreen!20}
ReToken (Single-pass) & 87.8 & 74.2 & 67.0 & 59.4 & 55.6 & 52.0 & 50.6 & 49.8 \\

\rowcolor{SeaGreen!20}
\textbf{ReToken (Two-pass)} &  87.8 & 85.9 & 84.4 & 82.5 & 80.7 & 76.8 & 72.0 & 67.7 \\

\bottomrule 
\end{tabular}
}
\end{table}
